Adversarial Networks for Spatial Context-Aware Spectral Image Reconstruction from RGB

Hyperspectral signal reconstruction aims at recovering the original spectral input that produced a certain trichromatic (RGB) response from a capturing device or observer. Given the heavily underconstrained, non-linear nature of the problem, traditional techniques leverage different statistical properties of the spectral signal in order to build informative priors from real world object reflectances for constructing such RGB to spectral signal mapping. However, most of them treat each sample independently, and thus do not benefit from the contextual information that the spatial dimensions can provide. We pose hyperspectral natural image reconstruction as an image to image mapping learning problem, and apply a conditional generative adversarial framework to help capture spatial semantics. This is the first time Convolutional Neural Networks -and, particularly, Generative Adversarial Networks- are used to solve this task. Quantitative evaluation shows a Root Mean Squared Error (RMSE) drop of 33.2% and a Relative RMSE drop of 54.0% on the ICVL natural hyperspectral image dataset.

==> resources_bmvc2017.tex <==
\begin{figure*}
	\begin{center}
		\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
	\end{center}
	\caption{Example of a short caption, which should be centered.}
	\label{fig:short}
\end{figure*}

%_________________________________________

\begin{table}
	\begin{center}
		\begin{tabular}{|l|c|}
			\hline
			Method & Frobnability \\
			\hline\hline
			Theirs & Frumpy \\
			Yours & Frobbly \\
			Ours & Makes one's heart Frob\\
			\hline
		\end{tabular}
	\end{center}
	\caption{Results.   Ours is better.}
\end{table}

%_________________________________________
\begin{figure}
	\begin{tabular}{ccc}
		\bmvaHangBox{\fbox{\parbox{2.7cm}{~\\[2.8mm]
					\rule{0pt}{1ex}\hspace{2.24mm}\includegraphics[width=2.33cm]{images/eg1_largeprint.png}\\[-0.1pt]}}}&
		\bmvaHangBox{\fbox{\includegraphics[width=2.8cm]{images/eg1_largeprint.png}}}&
		\bmvaHangBox{\fbox{\includegraphics[width=5.6cm]{images/eg1_2up.png}}}\\
		(a)&(b)&(c)
	\end{tabular}
	\caption{It is often a good idea for the first figure to attempt to
		encapsulate the article, complementing the abstract.  This figure illustrates
		the various print and on-screen layouts for which this paper format has
		been optimized: (a) traditional BMVC print format; (b) on-screen
		single-column format, or large-print paper; (c) full-screen two column, or
		2-up printing. }
	\label{fig:teaser}
\end{figure}
%_________________________________________
Saying ``this builds on the work of Lucy Smith [1]'' does not say
that you 

%_________________________________________
 {\em require} 
  using {\tt pdflatex},
  {\bf overlength will not be reviewed}. 
   useful {\em aide	memoire} in 
%_________________________________________
in~\cite{Authors06b}
shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is
a complete word.)  The provided \verb'\etal' macro is a useful {\em aide
	memoire} in this regard
We use {\tt natbib}, so citations in random order are nicely sorted:
\cite{Alpher03,Alpher02,Authors06b,Authors06}.  


%_________________________________________

ences (e.g.\ this line is $210.5$), although in
most cases one would expect that the approximate location ($210$ in the
previous example) will be adequate.

%_________________________________________


==> resources_iccv2017.tex <==
%\subsection{Paper length}
%For ICCV 2017, the rules about paper length have changed, so please read this section carefully. Papers, excluding the references section, must be %no longer than eight pages in length. There are no page limits for references.

%Mermin's description of how to write mathematics:
%\url{http://www.pamitc.org/documents/mermin.pdf}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

When placing figures in \LaTeX, it's almost always best to use
\verb+\includegraphics+, and to specify the  figure width as a multiple of
the line width as in the example below
{\small\begin{verbatim}
	\usepackage[dvips]{graphicx} ...
	\includegraphics[width=0.8\linewidth]
	{myfile.eps}
	\end{verbatim}
}

\begin{figure}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
\end{center}
   \caption{Example of caption.  It is set in Roman so that mathematics
   (always set in Roman: $B \sin A = A \sin B$) may be included without an
   ugly clash.}
\label{fig:long}
\label{fig:onecol}
\end{figure}


\begin{figure*}
	\begin{center}
		\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
	\end{center}
	\caption{Example of a short caption, which should be centered.}
	\label{fig:short}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table}
	\begin{center}
		\begin{tabular}{|l|c|}
			\hline
			Method & Frobnability \\
			\hline\hline
			Theirs & Frumpy \\
			Yours & Frobbly \\
			Ours & Makes one's heart Frob\\
			\hline
		\end{tabular}
	\end{center}
	\caption{Results.   Ours is better.}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
	\verb'$conf_a$' &  $conf_a$ \\
	\verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a
sentence-ending space. So \eg is correct, {\em e.g.} is not.  The provided
\verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'',
shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word.)
However, use it only when there are three or more authors.  Thus, the
following is correct: ``
Frobnication has been trendy lately.
It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...''
because reference~\cite{Alpher03} has just two authors.  If you use the
\verb'\etal' macro provided, then you need not worry about double periods
when used at the end of a sentence as in Alpher \etal.

For this citation style, keep multiple citations in numerical (not
chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
\cite{Alpher02,Alpher03,Authors14}.

